Safe Control under Uncertainty

Controller synthesis for hybrid systems that satisfy temporal specifications expressing various system properties is a challenging problem that has drawn the attention of many researchers. However, making the assumption that such temporal properties are deterministic is far from the reality. For example, many of the properties the controller has to satisfy are learned through machine learning techniques based on sensor input data. In this paper, we propose a new logic, Probabilistic Signal Temporal Logic (PrSTL), as an expressive language to define the stochastic properties, and enforce probabilistic guarantees on them. We further show how to synthesize safe controllers using this logic for cyber-physical systems under the assumption that the stochastic properties are based on a set of Gaussian random variables. One of the key distinguishing features of PrSTL is that the encoded logic is adaptive and changes as the system encounters additional data and updates its beliefs about the latent random variables that define the safety properties. We demonstrate our approach by synthesizing safe controllers under the PrSTL specifications for multiple case studies including control of quadrotors and autonomous vehicles in dynamic environments.

==> chance.tex <==
Chance constrained programs are well-studied problems in the optimization theory~\cite{ben2009robust,boyd2004convex}, and more recently, they have been used in stochastic control of cyber-physical systems~\cite{vitus2012stochastic,vitus2013probabilistic,lenz2015stochastic,blackmore2011chance}. 
We focus on the structure defined in equation~\eqref{eq:prob4} for our chance constrained optimization.
We are interested in finding a strategy $\uH$ in an MPC scheme to minimize a cost function $J(\xi^H)$, over a finite horizon trajectory.
%We focus on the following structure of chance constrained optimization, where we are interested in finding a strategy $\uH$ that similar to equation~\eqref{eq:mpc}, minimizes a cost function $J(\xi^H)$, over a finite horizon trajectory. 
However, in this formulation, the trajectory at every time step $\xi(t) = (x_t,u_t)$ must satisfy a probabilistic constraint.
%\begin{equation}
%\label{eq:chance}
%\begin{aligned}
%	 &\underset{\uH}{\text{minimize}}
%	& \quad &J(\xi^H(x_0, \uH))&\\
%	 &\text{subject to}
%	& \quad &P(\lambda_\alpha(\xi(t)) \leq 0 ) > 1-\epsilon & \\
%	& && \forall t\in\{0,\dotsc, H-1\}. &
%	\end{aligned}		
%\end{equation}
Here, $\lambda_{\alpha_t}$ is a stochastic function of a signal $\xi(t)$ at time $t$. 
%This stochastic function is parameterized by a random variable $\alpha$ drawn from a distribution $\mathcal{D}$.
One of the important challenges of chance optimization is there are no guarantees that the optimization in equation~\eqref{eq:prob4} is convex.
The convexity of the problem depends on the structure of the function $\lambda_{\alpha_t}$, and the distribution $\mathcal{D}$.

In this paper, we assume that our predicates are of two forms. Either the predicate is deterministic~\ie $\alpha_t$ is drawn from a Dirac distribution, and $\lambda_{\alpha_t}<0$ is a convex constraint, or:
\begin{equation}
\lambda_{\alpha_t}(\xi(t)) = {\alpha_t}^\top \xi_x(t)={\alpha_t}^\top x_t, \quad \alpha_t \sim \n(\mu_t,\Sigma_t).
\end{equation}
 
It is shown that for this structure of $\lambda_{\alpha_t}$, where $\lambda_{\alpha_t}$ is a weighted sum of the states with Gaussian weights $\alpha_t$, the chance constrained optimization in equation~\eqref{eq:prob4} is convex~\cite{van1963minimum,kataoka1963stochastic}.
This optimization, can be transformed to a second-order cone program (SOCP). 
The calculation is done by defining a standard Gaussian random variable $\nu \sim \n(0,1)$, which further allows us to use the Normal Cumulative Distribution Function (cdf):
\begin{equation}
\epsilon = \Phi (z) =  \int_{-\infty}^z \frac{1}{\sqrt{2\pi}}e^{\frac{-t^2}{2}}dt \quad \quad z = \Psi(\epsilon)	 = \Phi^{-1}(\epsilon).
\end{equation}
Here, $\Psi$ is the inverse of the Normal \emph{cdf} function, and is used in transforming the chance constraints to second-order cone constraints:
%\dorsa{Check the inequalities again}
\begin{equation}
\begin{aligned}
	&P(\lambda_{\alpha_t}(\xi(t)) < 0) > 1-{\epsilon_t}\\
	&\iff P(\alpha_t^\top x_t < 0) > 1-\epsilon_t \\
	&\iff P(\nu < \frac{-\mu_t^\top x_t}{x_t^\top \Sigma_t x_t}) > 1-\epsilon_t \\
	&\iff \int_{-\infty}^{\frac{-\mu_t^\top x_t}{x_t^\top \Sigma_t x_t}} \frac{1}{\sqrt{2\pi}} e^{\frac{-t^2}{2}} dt > 1-\epsilon_t \\
	&\iff \Phi(\frac{\mu_t^\top x_t}{x_t^\top \Sigma_t x_t}) < \epsilon_t \\
	&\iff \mu_t^\top x_t - \Psi(\epsilon_t) ||\Sigma_t^{1/2}x_t||_2  < 0
\end{aligned}	
\end{equation}
%More generally, we consider $\lambda_\alpha(\xt) = \alpha^\top f(\xt)$, where $f(\xt)$ is a convex function of $\xt$. 
%For our analysis of chance constrained optimizations, we impose the assumption that: $f(\xt) = \xt$.
%The chance constrained optimization in equation~\eqref{eq:chance}, with the specified structure of $\lambda_\alpha$, and Guassian $\alpha$, can be reformulated as a second order cone program (SOCP):
In this formulation, $\mu_t^\top x_t$ is the linear term, where $\mu_t$ is the mean of the random variable $\alpha_t$ at every time step, and $||\Sigma_t^{1/2}x_t||_2$ is the $l_2$-norm representing a quadratic term, where $\Sigma_t$ is the variance of $\alpha_t$. This quadratic term is scaled by $\Psi(\epsilon_t)$, the inverse of the Normal \emph{cdf} function, which is negative for small values of $\epsilon_t \leq 0.5$. 
So every chance constraint is reformulated as a SOCP, and as a result with a convex cost function $J(\xi^H)$, we can efficiently solve the following convex optimization for every predicate of \pstl:
\begin{equation}
\begin{aligned}
	 &\underset{\uH}{\text{minimize}}
	& \quad &J(\xi^H(x_0, \uH))&\\
	 &\text{subject to}
	&\quad  &\mu_t^\top x_t - \Psi(\epsilon_t) ||\Sigma_t^{1/2} x_t||_2< 0 &\\
	& & &\forall t\in\{0,\dotsc, H-1\}. &
	\end{aligned}		
\end{equation}
%\dorsa{Move this to the main section}
